Toward Quantum Simulations of $\mathbb{Z}_2$ Gauge Theory Without State Preparation

Preparing strongly-coupled particle states on quantum computers requires large resources. In this work, we show how classical sampling coupled with projection operators can be used to compute Minkowski matrix elements without explicitly preparing these states on the quantum computer. We demonstrate this for the 2+1d $\mathbb{Z}_2$ lattice gauge theory on small lattices with a quantum simulator.

==> imgs/conclusions.tex <==
%\documentclass[../main.tex]{subfiles}

%\begin{document}


\section{Conclusions}
\label{sec:con}

%\end{document}
